Diffusion-based Generative Prior for Low-Complexity MIMO Channel Estimation

This work proposes a novel channel estimator based on diffusion models (DMs), one of the currently top-rated generative models. Contrary to related works utilizing generative priors, a lightweight convolutional neural network (CNN) with positional embedding of the signal-to-noise ratio (SNR) information is designed by learning the channel distribution in the sparse angular domain. Combined with an estimation strategy that avoids stochastic resampling and truncates reverse diffusion steps that account for lower SNR than the given pilot observation, the resulting DM estimator has both low complexity and memory overhead. Numerical results exhibit better performance than state-of-the-art channel estimators utilizing generative priors.

==> befe.tex <==
\usepackage{xcolor}
\usepackage{hyperref}
% some of these options need the package xcolor
\hypersetup{
	colorlinks = true,
	% border around links like \eqref
	linkbordercolor = {white},
	% color of numbers in \cite
	citecolor = {black},
	% color of letters in links like \eqref
	linkcolor = {black},
	% color of letters in url
	urlcolor = {black}
}

\usepackage[acronym,shortcuts]{glossaries}
\glsdisablehyper %disable hyperlinks for abbreviations
\usepackage{amsmath,amssymb,amsthm,fixmath}
\usepackage{bm}
\usepackage{multicol}
\usepackage{float}
\usepackage{pgfplotstable}	
\usepackage{tikz}
\usetikzlibrary{shapes,arrows,positioning,calc}
\pgfplotsset{compat=1.18}
\usepackage{cleveref}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{url}


\RequirePackage{algorithm}
\RequirePackage{algorithmic}

\usepgfplotslibrary{statistics}
\usetikzlibrary{patterns}
\usetikzlibrary{decorations.pathmorphing,calc,shapes,shapes.geometric}
\usepgfplotslibrary{groupplots,dateplot}
\usetikzlibrary{patterns,shapes.arrows}
\usetikzlibrary{backgrounds,positioning,fit,matrix,fillbetween}


\newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}

\newcommand{\op}[1]{{\operatorname{#1}}}
\newcommand{\B}[1]{{\bm{#1}}}
\newcommand{\uproman}[1]{\uppercase\expandafter{\romannumeral#1}}
\newcommand{\E}{\operatorname{E}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\area}{\mathcal{Q}^{-1}}
\newcommand{\intall}{\int_{-\infty}^{\infty}}
\newcommand{\intC}{\int_{\mathbb{C}}}
\newcommand{\intR}{\int_{\mathbb{R}}}
\newcommand{\fhr}{f_{\B h|\B r}}
\newcommand{\fh}{f_{\B h}}
\newcommand{\frh}{p_{\B r|\B h}}
\newcommand{\fr}{p_{\B r}}
\newcommand{\dx}{\operatorname{d}\hspace{-1.5pt}}
\newcommand{\h}{^{\operatorname{H}}}
\newcommand{\T}{^{\operatorname{T}}}
\newcommand{\inv}{^{-1}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\nondiag}{\operatorname{nondiag}}
%\newcommand{\eye}{\B I}
\DeclareMathOperator{\eye}{\mathbf{I}}
\DeclareMathOperator{\dft}{\mathbf{F}}
\newcommand{\vect}{\operatorname{vec}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\sqrtm}{^{-\frac{1}{2}}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Qinv}{\overline{Q}}
\newcommand{\erf}{\operatorname{erf}}
\newcommand{\fft}{\operatorname{fft}}
\newcommand{\ifft}{\operatorname{ifft}}
\newcommand{\rr}{r_{\Re}}
\newcommand{\hr}{h_\Re}
\newcommand{\nr}{n_\Re}
\newcommand{\brr}{\B r_\Re}
\newcommand{\bhr}{\B h _\Re}
\newcommand{\NC}{\mathcal{N}_{\C}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\DKL}{\op D_{\text{KL}}}
\newcommand{\balpha}{\bar{\alpha}}

\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
%\newcommand{\tinit}{{t_{\text{init}}}}
\newcommand{\tinit}{{\hat{t}}}
\newcommand{\limT}{\lim_{T\to\infty}}
\newcommand{\hhat}{\hat{\B h}}
\newcommand{\btheta}{{\B \theta}}

\newcommand{\Nrx}{{N_{\text{rx}}}}
\newcommand{\Ntx}{{N_{\text{tx}}}}

% plot sizes
\newcommand{\plotwidth}{0.98\columnwidth}
\newcommand{\plotheight}{0.6\columnwidth}

\newcommand{\plotwidthapp}{0.98\columnwidth}
\newcommand{\plotheightapp}{0.6\columnwidth}

% line styles
\newcommand{\lineWidth}{1.0pt}
\newcommand{\marksize}{2.2pt}

\pgfplotsset{every axis/.append style={
                    %axis x line=middle,    % put the x axis in the middle
                    %axis y line=middle,    % put the y axis in the middle
                    %axis line style={<->}, % arrows on the axis
                    %xlabel={$x$},          % default put x on x-axis
                    %ylabel={$y$},          % default put y on y-axis
                    label style={font=\scriptsize},
                    tick label style={font=\scriptsize}  
                    }}



\newacronym{awgn}{AWGN}{additive white Gaussian noise}
\newacronym{dm}{DM}{diffusion model}
\newacronym{nn}{NN}{neural network}
\newacronym{snr}{SNR}{signal-to-noise ratio}
\newacronym{elbo}{ELBO}{evidence lower bound}
\newacronym{cme}{CME}{conditional mean estimator}
\newacronym{vae}{VAE}{variational autoencoder}
\newacronym{gan}{GAN}{generative adversarial network}
\newacronym{gpt}{GPT}{generative pre-trained transformer}
\newacronym{mse}{MSE}{mean square error}
\newacronym{mfa}{MFA}{mixture of factor analyzer}
%\newacronym{mmse}{MMSE}{minimum mean square error}
\newacronym{pdf}{PDF}{probability density function}
\newacronym{kl}{KL}{Kullback–Leibler}
\newacronym{psnr}{PSNR}{peak signal-to-noise ratio}
\newacronym{gmm}{GMM}{Gaussian mixture model}
\newacronym{silu}{SiLU}{sigmoid linear unit}
\newacronym{ls}{LS}{least squares}
\newacronym{stft}{STFT}{short-time Fourier transform}
% \newacronym{gpu}{GPU}{graphics processing unit}
\newacronym{cnn}{CNN}{convolutional neural network}
\newacronym{bs}{BS}{base station}
\newacronym{mt}{MT}{mobile terminal}
\newacronym{mmse}{MMSE}{minimum mean square error}
\newacronym{omp}{OMP}{orthogonal matching pursuit}
\newacronym{mimo}{MIMO}{multiple-input multiple-output}
\newacronym{dft}{DFT}{discrete Fourier transform}
\newacronym{fft}{FFT}{fast Fourier transform}
\newacronym{3gpp}{3GPP}{3rd Generation Partnership Project}
\newacronym{los}{LOS}{line-of-sight}
\newacronym{relu}{ReLU}{rectified linear unit}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}


\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
